Design Guidelines for Improving User Experience in Industrial Domain-Specific Modelling Languages

Domain-specific modelling languages (DSMLs) help practitioners solve modelling challenges specific to various domains. As domains grow more complex and heterogeneous in nature, industrial practitioners often face challenges in the usability of graphical DSMLs. There is still a lack of guidelines that industrial language engineers should consider for improving the user experience (UX) of these practitioners. The overall topic of UX is vast and subjective, and general guidelines and definitions of UX are often overly generic or tied to specific technological spaces. To solve this challenge, we leverage existing design principles and standards of human-centred design and UX in general and propose definitions and guidelines for UX and user experience design (UXD) aspects in graphical DSMLs. In this paper, we categorize the key UXD aspects, primarily based on our experience in developing industrial DSMLs, that language engineers should consider during graphical DSML development. Ultimately, these UXD guidelines help to improve the general usability of industrial DSMLs and support language engineers in developing better DSMLs that are independent of graphical modelling tools and more widely accepted by their users.

==> 05_Example.tex <==
\section{Example/Demonstration (1.5p)}
\label{sec:demos}

With screenshots, needs more space?

Introduce the UXD aspects using different DSL examples.

SpesML?

==> 08_Acknowledgement.tex <==
\begin{acknowledgments}
\label{sec:ack}
	Ack goes here.
\end{acknowledgments}



